Assessing Quality Metrics for Neural Reality Gap Input Mitigation in Autonomous Driving Testing

Simulation-based testing of automated driving systems (ADS) is the industry standard, being a controlled, safe, and cost-effective alternative to real-world testing. Despite these advantages, virtual simulations often fail to accurately replicate real-world conditions like image fidelity, texture representation, and environmental accuracy. This can lead to significant differences in ADS behavior between simulated and real-world domains, a phenomenon known as the sim2real gap. Researchers have used Image-to-Image (I2I) neural translation to mitigate the sim2real gap, enhancing the realism of simulated environments by transforming synthetic data into more authentic representations of real-world conditions. However, while promising, these techniques may potentially introduce artifacts, distortions, or inconsistencies in the generated data that can affect the effectiveness of ADS testing. In our empirical study, we investigated how the quality of image-to-image (I2I) techniques influences the mitigation of the sim2real gap, using a set of established metrics from the literature. We evaluated two popular generative I2I architectures, pix2pix, and CycleGAN, across two ADS perception tasks at a model level, namely vehicle detection and end-to-end lane keeping, using paired simulated and real-world datasets. Our findings reveal that the effectiveness of I2I architectures varies across different ADS tasks, and existing evaluation metrics do not consistently align with the ADS behavior. Thus, we conducted task-specific fine-tuning of perception metrics, which yielded a stronger correlation. Our findings indicate that a perception metric that incorporates semantic elements, tailored to each task, can facilitate selecting the most appropriate I2I technique for a reliable assessment of the sim2real gap mitigation.

==> 2-background.tex <==
% !TEX root =  paper.tex
% \section{Background}\label{sec:background}

% \subsection{ADS Testing}

% \head{Autonomous Vehicles}

% Current ADS are equipped with a multitude of sensors (such as cameras, LIDAR, and GPS) to perform different prediction and control tasks, such as lane keeping, object detection, object avoidance, and path planning~\cite{yurtsever2020survey,chen2023endtoend}. The information collected by the sensors during the data collection campaign is used to train advanced DNNs to predict control values that are sent to the vehicle actuators to perform the driving maneuvers (e.g., steering or braking). 

% % \head{Testing Levels for Autonomous Vehicles}

% Validating the capabilities and reliability of ADS is a highly complex task. To validate the safety of ADS, automakers adopt a multi-pillar approach including simulation/virtual testing, test track, and real-world testing~\cite{waymos-secret-testing,Cerf:2018:CSC:3181977.3177753}. 
% %
% Simulation/virtual testing uses simulation toolkits to assess the compliance of an ADS with the safety requirements on a wide range of virtual scenarios, some of which are extremely difficult if not impossible to encounter and test in the real world. Track testing uses a closed-access testing ground with various scenario elements to test the functioning of an ADS in a physical environment. Finally, the last pillar involves real-world testing on public roads, to evaluate the capabilities of the ADS to drive safely in everyday real-life conditions (e.g., traffic).

% In our work, we study system-level testing of SDC models that perform \textit{behavioral cloning}, i.e., the autopilot learns the \textit{lane keeping} functionality from a dataset of driving scenes collected from a human driver.
% Our focus is on the comparison between virtual and physical closed-loop track testing. In the rest of the paper, we shall use the terms virtual/digital/simulated, as well as the terms physical/real-world, interchangeably). 

% While real-world sensor data of the vehicle are recorded and recreated within the simulator, ensuring the safety, effectiveness, and transferability of ADS testing in the real world is still an open challenge. 

% \subsection{sim2real}

% TODO  1
% \head{Generative Models}\label{sec:i2i}
% %
% Generative models represent a class of machine learning models designed to produce novel data resembling a provided dataset. This is achieved by capturing the underlying patterns and structures within the data, enabling the generation of novel data samples.
% Among these methods, Generative Adversarial Networks (GANs)~\cite{NIPS2014_5423} have emerged as the most popular solution. GANs consist of two neural networks, namely the Generator and the Discriminator, that engage in a competitive learning process known as adversarial learning. The Generator's objective is to create synthetic data that is indistinguishable from real samples, while the Discriminator learns to accurately differentiate between them.

% In the context of autonomous driving, GANs have been applied to various tasks such as input pre-processing, including raindrop removal~\cite{de_rain_1}, de-blurring~\cite{de_blur}, and de-hazing~\cite{de_haze}. They also found applications in sim2real I2I translation tasks~\cite{2023-Stocco-TSE,deeproad,sim2real_gans_cit,sim2real_gans_cit_2}, in which one significant challenge is ensuring that the generated images not only look realistic but also preserve the essential content and details of the input, i.e., their \textit{semantics}. Since adversarial training may not guarantee semantics preservation, researchers have proposed GAN variations that introduce constraints on the Generator's output. Instances of these solutions are pix2pix~\cite{pix2pix}, UNIT~\cite{unit}, DiscoGAN~\cite{disco_gan}, and CycleGAN~\cite{cyclegan}.

% TODO 2

% \head{Issues of Generative Models}\label{sec:I2I_shortcomings}
% %
% Researchers have identified issues within GANs, including I2I models, that could potentially affect systems reliant on the use of their generated images as input. These include visual anomalies such as color bleeding, feature blending, omission, hallucination, erroneous object textures, and pixel patterns which can introduce inaccuracies and inconsistencies, disrupting ADS related to object recognition, segmentation, and scene understanding tasks~\cite{gan_problems_1}. 

% The objective of this study is to explore the advantages and drawbacks of employing I2I models for sim2real gap mitigation in the context of ADS testing. Our specific goals are twofold. First, we aim to assess whether the effectiveness of I2I models can be transferred to various ADS tasks or if certain I2I solutions are better suited for specific ones. Second, we aim to assess whether the existing metrics used to evaluate the quality of I2I model outputs are correlated with the performance of the ADS being tested and whether improvements to the existing metrics can be made. 





==> 5-discussion.tex <==
% !TEX root =  paper.tex
\section{Discussion}\label{sec:discussion}

\head{I2I model selection}
%
Our study revealed that I2I gap mitigation performance is not maintained across different task domains. While I2I models can enhance image quality and bridge the simulation-to-reality gap to some extent, their usage in a production setting is still a careful choice, which necessitates a deep understanding of the ADS task.
% This finding underscores the critical importance of selecting the most suitable I2I model for a specific task. 
% It is evident that not all models perform uniformly well across diverse domains, therefore, making the right choice is crucial to ensure effective gap mitigation. While these models can enhance image quality and bridge the simulation-to-reality gap, our results indicate that their effectiveness can vary. This necessitates a thoughtful and context-specific approach to their use.
\head{\\Domain-level vs single-image metrics}
% Our results indicate that domain-level metrics tend to exhibit correlations with ADS behavior, but are inconsistent across domains. With an attentive metric selection tailored to the evaluated task, they can be useful as a training measure for I2I models.
Our study highlighted that domain-level metrics exhibit good correlations with the ADS behavior, however with poor consistency across domains. Provided a careful metric selection for a given task, these metrics can be used during the training of I2I models. Nonetheless, their inability to assess single images individually makes them less suitable for testing purposes. %, especially for the validation of individual samples and corner cases.
In contrast, single-image metrics are better suited for evaluating individual images, but our findings indicate their limited reliability across the vehicle detection and lane-keeping domains. 
\head{\\Single-image metrics fine-tuning and usage}
The observations obtained in RQ\textsubscript{2} highlight the need for task-specific tuning of the existing metrics.
The development of our proposed perception-based single-image metric was driven by the intuition that fine-tuning a task-specific metric on ADS domain would reinforce its correlation with the ADS that uses them. This result was confirmed experimentally. 
We opted to employ a pixel segmentation model, as segmentation is a universally applicable concept for imagery data for describing high-level semantics. 
Our results align with our expectations, as demonstrated by our proposed \onemetric metric. In terms of model prediction error, this metric stands out as the only one observed to exhibit strong correlations with images generated by different I2I architectures across two distinct task domains.





